Verifiable Sustainability in Data Centers

Data centers have significant energy needs, both embodied and operational, affecting sustainability adversely. The current techniques and tools for collecting, aggregating, and reporting verifiable sustainability data are vulnerable to cyberattacks and misuse, requiring new security and privacy-preserving solutions. This paper outlines security challenges and research directions for addressing these pressing requirements.

==> Makefile <==
NAME=main
SRC=$(wildcard *.tex */*.tex)

BIB=$(wildcard *.bib */*.bib)
STY=$(wildcard *.sty *.cls)

FIGS=$(wildcard figures/*.pdf)

$(NAME).pdf: $(SRC) $(BIB) $(STY) $(FIGS) $(wildcard *.yaml)
	pdflatex $(NAME)
	bibtex $(NAME)
	pdflatex $(NAME)
	bibtex $(NAME)
	pdflatex $(NAME)

getbib: $(HOME)/tex/bib/master.bib $(HOME)/tex/bib/fsl-macros.tex $(HOME)/tex/bib/acmart.cls
	(cd $(HOME)/tex/bib && cvs update)
	-mkdir -p template
	cp -av $(HOME)/tex/bib/fsl-macros.tex template
	cp -av $(HOME)/tex/bib/master.bib template
#	cp -av $(HOME)/tex/bib/acmart.cls .

# Erez rules to facilitate easier reviewing via diffs
ezdiff:
	-mv -f diffs.txt diffs.txt.old
	-chmod u+w diffs.txt.old
	-ezgit diff `lsr-tex $(NAME)` Makefile $(BIB) > diffs.txt
	chmod 444 diffs.txt
	diffstat diffs.txt

show: $(NAME).pdf
	open $?

check:
	perl ${HOME}/proj/fsl/bib/consistify ${SRCS} ${SRC}

clean: FRC
	$(RM) $(RMFLAGS) *~ .*~ \#* core
	$(RM) $(RMFLAGS) *.dvi $(NAME).ps temp.ps *.lj *.lj4 $(NAME).bbl
	$(RM) $(RMFLAGS) $(NAME).ttt $(NAME).fff $(NAME).pdf $(NAME).txt
	$(RM) $(RMFLAGS) *.log *.aux *.toc *.lof *.blg *.lot *.cb $(NAME).out
	$(RM) $(RMFLAGS) slides2.ps slides4.ps *.bibdiff

FRC:

